Verification of indefinite-horizon POMDPs

The verification problem in MDPs asks whether, for any policy resolving the nondeterminism, the probability that something bad happens is bounded by some given threshold. This verification problem is often overly pessimistic, as the policies it considers may depend on the complete system state. This paper considers the verification problem for partially observable MDPs, in which the policies make their decisions based on (the history of) the observations emitted by the system. We present an abstraction-refinement framework extending previous instantiations of the Lovejoy-approach. Our experiments show that this framework significantly improves the scalability of the approach.

==> abstractions.tex <==
%!TEX root = main.tex
% !TeX spellcheck = en_GB
\section{Belief Abstraction}
{\color{gray}
\tq{this section is probably obsolete}

%\tq{A belief decomposition is not an equivalence relation: Grid points belong to multiple classes.}
\begin{definition}[Belief Abstraction]
	Let  $\pomdp = \pomdptuple$ be a POMDP with $\numstates$ states and belief MPD $\beliefmdp{\pomdp} = \tuple{\beliefstates, \actions, \belieftransitions, \binit}$.
	A \emph{belief abstraction} is an equivalence relation $\belabs$ on $\beliefstates$ such that
	\begin{itemize}
		\item the equivalence class $\classof{\beliefstate} = \set{\beliefstate' \in \beliefstates \mid \tuple{\beliefstate,\beliefstate'} \in \belabs}$ is an (open or closed) polytope for all $\beliefstate \in \beliefstates$, and
		\item $\tuple{\beliefstate,\beliefstate'} \in \belabs$ implies $\obsof{\beliefstate} = \obsof{\beliefstate'}$.
	\end{itemize}
\end{definition}
The equivalence classes of the coarsest possible belief abstraction is given by the sets of belief states with the same observation.
Let $\belabs$ be a belief abstraction.
We say $\belabs$ is finite, if it has a finite index, \ie the set $\set{\classof{\beliefstate} \mid \beliefstate \in \beliefstates}$ is finite.
For each equivalence class $\classof{\beliefstate}$ we fix one representant, denoted by $\reprof{\classof{\beliefstate}} \in \classof{\beliefstate}$. For simplicity, we may also write $\reprof{\beliefstate}$.
For example, this could be the center point of the polytope $\classof{\beliefstate}$.
The set of \emph{representants} for $\belabs$ is given by the union of all representatives, \ie $\representants = \bigcup_{\beliefstate \in \beliefstates} \reprof{\beliefstate}$.
The set of \emph{intersections} for $\belabs$ is given by the union of the vertices of all equivalence classes, \ie $\intersections = \bigcup_{\beliefstate \in \beliefstates} \vertices{\classof{\beliefstate}}$
Both, $\representants$ and $\intersections$ are subsets of the set of belief states.
If $\belabs$ is finite, $\representants$ and $\intersections$ are finite.


\begin{definition}[Under-approximation]
	The under-approximation for POMDP $\pomdptuple$ with underlying MDP $\mdp=\mdptuple$, belief MDP $\beliefmdp{\pomdp} = \tuple{\beliefstates, \actions, \belieftransitions, \binit}$, and belief abstraction $\belabs$ is given by the MDP $\undermdp{\pomdp}{\belabs} = \tuple{\representants, \actions, \transitions_\belabs, \reprof{\sinit}}$, where for all $\repr, \repr' \in \representants, \action \in \act{\repr}$ transitions are defined as follows:
	\[
	\transitions_\belabs(\repr, \action, \repr') = \sum_{\beliefstate' \in \post[\beliefmdp{\mdp}]{\repr}{\action}}
	 \iverson{\reprof{\beliefstate'} = \repr'} \cdot \belieftransitions(\repr, \action, \beliefstate')
	\]
\end{definition}

\begin{theorem}
	It's really an under approximation for reachability probabilities.
\end{theorem}
\begin{proof}
	A positional strategy for $\undermdp{\pomdp}{\belabs}$ is easily mapped to a positional strategy for $\beliefmdp{\mdp}$.
\end{proof}

For the over-approximation we observe that every belief state $\beliefstate$ can be represented by a convex combination of the vertices $\vertices{\classof{\beliefstate}}$.
We associate to each $\beliefstate \in \beliefstates$ a distribution $\dist_{\beliefstate} \in \dists{\vertices{\classof{\beliefstate}}}$ such that $\beliefstate = \sum_{\vertex \in \vertices{\classof{\beliefstate}}} \dist_{\beliefstate}(\vertex) \cdot \vertex$.
\begin{definition}[Over-approximation]
	The over-approximation for POMDP $\pomdptuple$ with underlying MDP $\mdp=\mdptuple$, belief MDP $\beliefmdp{\pomdp} = \tuple{\beliefstates, \actions, \belieftransitions, \binit}$, and belief abstraction $\belabs$ is given by the MDP $\overmdp{\pomdp}{\belabs} = \tuple{\intersections \cup \set{\inter_{\mathit{I}}}, \actions, \transitions^\belabs, \inter_{\mathit{I}}}$, where for all $\inter, \inter' \in \intersections$
\end{definition}
}


==> experiments/fixed.tex <==
\begin{tabular}{|cc|rrr|r|r|r|r|r|r|r|r|r|r|}
\hline
\multicolumn{2}{|c|}{Benchmark} & \multicolumn{3}{c|}{Data} & MDP & u=60 & \multicolumn{3}{c|}{g=04} & \multicolumn{3}{c|}{g=12} & r=0060 & r=1800\\
Model & Prop & States & Obs & Act & \multicolumn{2}{c|}{storm} & prism & \multicolumn{2}{c|}{storm} & prism & \multicolumn{4}{c|}{storm}\\
 &  &  &  &  &  &  &  & t=0 & t=0.2 &  & t=0 & t=0.2 &  & \\
\hline
crypt & \multirow{2}{*}{Pmax} & \multirow{2}{*}{$275$} & \multirow{2}{*}{$130$} & \multirow{2}{*}{$499$} & \multirow{2}{*}{1} & $\ge 0.5$ & $[0.5, 0.5]$ & $\le 0.5$ & $\le 0.5$ & $[0.5, 0.5]$ & $\le 0.5$ & $\le 0.5$ & $\le 0.5$ & $\le 0.5$\\
N3 &  &  &  &  &  & 2* / $148$ & \ensuremath{3.32} / $1046$ & \ensuremath{< 1} / $116$ & \ensuremath{< 1} / $116$ & \ensuremath{3.84} / $8542$ & \ensuremath{1.14} / $116$ & \ensuremath{< 1} / $116$ & 3* / $140$ & 3* / $140$\\
\hline
crypt & \multirow{2}{*}{Pmin} & \multirow{2}{*}{$275$} & \multirow{2}{*}{$130$} & \multirow{2}{*}{$499$} & \multirow{2}{*}{0} & $\le 0.5$ & $[0.5, 0.5]$ & $\ge 0.5$ & $\ge 0.5$ & $[0.5, 0.5]$ & $\ge 0.5$ & $\ge 0.5$ & $\ge 0.5$ & $\ge 0.5$\\
N3 &  &  &  &  &  & 2* / $148$ & \ensuremath{2.86} / $1046$ & \ensuremath{< 1} / $116$ & \ensuremath{< 1} / $116$ & \ensuremath{3.58} / $8542$ & \ensuremath{< 1} / $116$ & \ensuremath{1.06} / $116$ & 27* / $116$ & 27* / $116$\\
\hline
crypt & \multirow{2}{*}{Pmax} & \multirow{2}{*}{$1972$} & \multirow{2}{*}{$510$} & \multirow{2}{*}{$4612$} & \multirow{2}{*}{1} & $\ge 0.333$ & $[0.333, 0.792]$ & $\le 0.667$ & $\le 0.667$ &  & $\le 0.333$ & $\le 0.333$ & $\le 0.333$ & $\le 0.333$\\
N4 &  &  &  &  &  & 2* / $912$ & \ensuremath{17.3} / $5{\cdot} 10^{4}$ & \ensuremath{1.14} / $1044$ & \ensuremath{< 1} / $1044$ & MO / $3{\cdot} 10^{7}$ & \ensuremath{1.09} / $464$ & \ensuremath{< 1} / $464$ & 27* / $464$ & 27* / $464$\\
\hline
crypt & \multirow{2}{*}{Pmin} & \multirow{2}{*}{$1972$} & \multirow{2}{*}{$510$} & \multirow{2}{*}{$4612$} & \multirow{2}{*}{0} & $\le 0.333$ & $[0, 0.333]$ & $\ge 0.083$ & $\ge 0.083$ &  & $\ge 0.333$ & $\ge 0.333$ & $\ge 0.333$ & $\ge 0.333$\\
N4 &  &  &  &  &  & 2* / $912$ & \ensuremath{17.9} / $5{\cdot} 10^{4}$ & \ensuremath{< 1} / $1044$ & \ensuremath{1.18} / $1044$ & MO / $3{\cdot} 10^{7}$ & \ensuremath{1.18} / $464$ & \ensuremath{1.18} / $464$ & 31 / $608$ & 32 / $1168$\\
\hline
crypt & \multirow{2}{*}{Pmax} & \multirow{2}{*}{$1{\cdot} 10^{4}$} & \multirow{2}{*}{$1882$} & \multirow{2}{*}{$4{\cdot} 10^{4}$} & \multirow{2}{*}{1} & $\ge 0.25$ &  & $\le 1$ & $\le 1$ &  & $\le 0.667$ & $\le 0.667$ & $\le 0.25$ & $\le 0.25$\\
N5 &  &  &  &  &  & 2* / $2012$ & TO / $2{\cdot} 10^{6}$ & \ensuremath{< 1} / $9028$ & \ensuremath{< 1} / $9028$ & MO / N/A & \ensuremath{< 1} / $1{\cdot} 10^{4}$ & \ensuremath{< 1} / $1{\cdot} 10^{4}$ & 13* / $3868$ & 13* / $3868$\\
\hline
crypt & \multirow{2}{*}{Pmin} & \multirow{2}{*}{$1{\cdot} 10^{4}$} & \multirow{2}{*}{$1882$} & \multirow{2}{*}{$4{\cdot} 10^{4}$} & \multirow{2}{*}{0} & $\le 0.25$ &  & $\ge 0$ & $\ge 0$ &  & $\ge 0$ & $\ge 0$ & $\ge 0.25$ & $\ge 0.25$\\
N5 &  &  &  &  &  & 2* / $2012$ & TO / $2{\cdot} 10^{6}$ & \ensuremath{1.51} / $9028$ & \ensuremath{< 1} / $9028$ & MO / N/A & \ensuremath{< 1} / $1{\cdot} 10^{4}$ & \ensuremath{< 1} / $1{\cdot} 10^{4}$ & 21* / $2092$ & 21* / $2092$\\
\hline
crypt & \multirow{2}{*}{Pmax} & \multirow{2}{*}{$7{\cdot} 10^{4}$} & \multirow{2}{*}{$6678$} & \multirow{2}{*}{$2{\cdot} 10^{5}$} & \multirow{2}{*}{1} & $\ge 0.2$ &  & $\le 1$ & $\le 1$ &  & $\le 0.717$ & $\le 0.717$ & $\le 0.964$ & $\le 0.2$\\
N6 &  &  &  &  &  & 2* / $2{\cdot} 10^{4}$ & MO / N/A & \ensuremath{10.7} / $8{\cdot} 10^{4}$ & \ensuremath{10.8} / $8{\cdot} 10^{4}$ & MO / N/A & \ensuremath{9.31} / $7{\cdot} 10^{4}$ & \ensuremath{9.34} / $7{\cdot} 10^{4}$ & 3 / $2{\cdot} 10^{5}$ & 17* / $2{\cdot} 10^{4}$\\
\hline
crypt & \multirow{2}{*}{Pmin} & \multirow{2}{*}{$7{\cdot} 10^{4}$} & \multirow{2}{*}{$6678$} & \multirow{2}{*}{$2{\cdot} 10^{5}$} & \multirow{2}{*}{0} & $\le 0.2$ &  & $\ge 0$ & $\ge 0$ &  & $\ge 0$ & $\ge 0$ & $\ge 0$ & $\ge 0.2$\\
N6 &  &  &  &  &  & 2* / $2{\cdot} 10^{4}$ & MO / N/A & \ensuremath{10.3} / $8{\cdot} 10^{4}$ & \ensuremath{4.8} / $3$ & MO / N/A & \ensuremath{9.09} / $7{\cdot} 10^{4}$ & \ensuremath{4.8} / $3$ & 3 / $2{\cdot} 10^{5}$ & 28* / $6360$\\
\hline
drone & \multirow{2}{*}{Pmax} & \multirow{2}{*}{$497$} & \multirow{2}{*}{$228$} & \multirow{2}{*}{$1172$} & \multirow{2}{*}{0.961} & $\ge 0.86$ &  & $\le 0.927$ & $\le 0.927$ &  & $\le 0.898$ & $\le 0.898$ & $\le 0.905$ & $\le 0.905$\\
N3 &  &  &  &  &  & 9 / $2{\cdot} 10^{6}$ & NS / N/A & \ensuremath{1.24} / $1{\cdot} 10^{4}$ & \ensuremath{< 1} / $1{\cdot} 10^{4}$ & NS / N/A & \ensuremath{14.6} / $5{\cdot} 10^{5}$ & \ensuremath{14.6} / $5{\cdot} 10^{5}$ & 4 / $4{\cdot} 10^{5}$ & 5$^\dagger$ / $3{\cdot} 10^{6}$\\
\hline
drone & \multirow{2}{*}{Pmax} & \multirow{2}{*}{$1226$} & \multirow{2}{*}{$761$} & \multirow{2}{*}{$2954$} & \multirow{2}{*}{0.983} & $\ge 0.952$ &  & $\le 0.977$ & $\le 0.977$ &  & $\le 0.974$ & $\le 0.974$ & $\le 0.976$ & $\le 0.975$\\
N4 &  &  &  &  &  & 7 / $1{\cdot} 10^{6}$ & NS / N/A & \ensuremath{< 1} / $3{\cdot} 10^{4}$ & \ensuremath{1.71} / $3{\cdot} 10^{4}$ & NS / N/A & \ensuremath{150} / $3{\cdot} 10^{6}$ & \ensuremath{150} / $3{\cdot} 10^{6}$ & 3 / $2{\cdot} 10^{5}$ & 4$^\dagger$ / $2{\cdot} 10^{6}$\\
\hline
drone & \multirow{2}{*}{Pmax} & \multirow{2}{*}{$2557$} & \multirow{2}{*}{$1215$} & \multirow{2}{*}{$6232$} &  & $\ge 0.888$ &  & $\le 0.988$ & $\le 0.988$ &  &  &  & $\le 0.988$ & $\le 0.988$\\
N5 &  &  &  &  &  & 5 / $1{\cdot} 10^{6}$ & NS / N/A & \ensuremath{13.6} / $4{\cdot} 10^{5}$ & \ensuremath{13.5} / $4{\cdot} 10^{5}$ & NS / N/A & MO / N/A & MO / N/A & 2 / $3{\cdot} 10^{5}$ & 3$^\dagger$ / $2{\cdot} 10^{6}$\\
\hline
drone & \multirow{2}{*}{Pmax} & \multirow{2}{*}{$4754$} & \multirow{2}{*}{$2818$} & \multirow{2}{*}{$1{\cdot} 10^{4}$} &  & $\ge 0.417$ &  & $\le 0.996$ & $\le 0.996$ &  &  &  & $\le 0.996$ & $\le 0.996$\\
N6 &  &  &  &  &  & 3 / $6{\cdot} 10^{5}$ & NS / N/A & \ensuremath{31.1} / $9{\cdot} 10^{5}$ & \ensuremath{33.8} / $9{\cdot} 10^{5}$ & NS / N/A & MO / N/A & MO / N/A & 2 / $5{\cdot} 10^{5}$ & 3$^\dagger$ / $6{\cdot} 10^{6}$\\
\hline
drone & \multirow{2}{*}{Pmax} & \multirow{2}{*}{$8129$} & \multirow{2}{*}{$3984$} & \multirow{2}{*}{$2{\cdot} 10^{4}$} &  & $\ge 0.337$ &  & $\le 0.998$ & $\le 0.998$ &  &  &  & $\le 0.998$ & $\le 0.998$\\
N7 &  &  &  &  &  & 2 / $8{\cdot} 10^{5}$ & NS / N/A & \ensuremath{345} / $6{\cdot} 10^{6}$ & \ensuremath{312} / $6{\cdot} 10^{6}$ & NS / N/A & MO / N/A & MO / N/A & 1 / $8{\cdot} 10^{5}$ & 2$^\dagger$ / $3{\cdot} 10^{6}$\\
\hline
drone & \multirow{2}{*}{Pmax} & \multirow{2}{*}{$1{\cdot} 10^{4}$} & \multirow{2}{*}{$7577$} & \multirow{2}{*}{$3{\cdot} 10^{4}$} &  & $\ge 0.276$ &  & $\le 0.999$ & $\le 0.999$ &  &  &  & $\le 0.999$ & $\le 0.999$\\
N8 &  &  &  &  &  & 1 / $7{\cdot} 10^{5}$ & NS / N/A & \ensuremath{759} / $1{\cdot} 10^{7}$ & \ensuremath{712} / $1{\cdot} 10^{7}$ & NS / N/A & MO / N/A & MO / N/A & 1 / $1{\cdot} 10^{6}$ & 2$^\dagger$ / $4{\cdot} 10^{6}$\\
\hline
grid & \multirow{2}{*}{Rmin} & \multirow{2}{*}{$17$} & \multirow{2}{*}{$3$} & \multirow{2}{*}{$62$} & \multirow{2}{*}{3.2} & $\le 4.133$ & $[3.596, 4.133]$ & $\ge 3.633$ & $\ge 3.633$ &  & $\ge 4.083$ & $\ge 4.083$ & $\ge 4.133$ & $\ge 4.133$\\
4x4 &  &  &  &  &  & 6* / $2423$ & \ensuremath{1.86} / $3061$ & \ensuremath{< 1} / $517$ & \ensuremath{< 1} / $517$ & MO / $1{\cdot} 10^{7}$ & \ensuremath{< 1} / $2880$ & \ensuremath{< 1} / $2880$ & 5* / $891$ & 5* / $891$\\
\hline
grid & \multirow{2}{*}{Rmin} & \multirow{2}{*}{$17$} & \multirow{2}{*}{$3$} & \multirow{2}{*}{$62$} & \multirow{2}{*}{3.556} & $\le 4.732$ & $[4.06, 4.702]$ & $\ge 4.06$ & $\ge 4.06$ &  & $\ge 4.588$ & $\ge 4.588$ & $\ge 4.558$ & $\ge 4.653$\\
4x4-sl &  &  &  &  &  & 13 / $1{\cdot} 10^{6}$ & \ensuremath{2.12} / $3061$ & \ensuremath{< 1} / $1655$ & \ensuremath{< 1} / $1655$ & MO / $1{\cdot} 10^{7}$ & \ensuremath{582} / $7{\cdot} 10^{6}$ & \ensuremath{593} / $7{\cdot} 10^{6}$ & 3 / $2{\cdot} 10^{5}$ & 4$^\dagger$ / $6{\cdot} 10^{6}$\\
\hline
grid-av & \multirow{2}{*}{Pmax} & \multirow{2}{*}{$17$} & \multirow{2}{*}{$4$} & \multirow{2}{*}{$59$} & \multirow{2}{*}{1} & $\ge 0.929$ & $[0.214, 1.0]$ & $\le 1$ & $\le 1$ &  & $\le 0.94$ & $\le 0.94$ & $\le 0.929$ & $\le 0.929$\\
4x4 &  &  &  &  &  & 8* / $9016$ & \ensuremath{1.37} / $2382$ & \ensuremath{< 1} / $272$ & \ensuremath{< 1} / $272$ & MO / $5{\cdot} 10^{6}$ & \ensuremath{< 1} / $4943$ & \ensuremath{< 1} / $4943$ & 6* / $2976$ & 6* / $2976$\\
\hline
grid-av & \multirow{2}{*}{Pmax} & \multirow{2}{*}{$17$} & \multirow{2}{*}{$4$} & \multirow{2}{*}{$59$} & \multirow{2}{*}{1} & $\ge 0.927$ & $[0.214, 1.0]$ & $\le 1$ & $\le 1$ &  & $\le 0.944$ & $\le 0.944$ & $\le 0.944$ & $\le 0.944$\\
4x4-sl &  &  &  &  &  & 13 / $1{\cdot} 10^{6}$ & \ensuremath{2.41} / $2382$ & \ensuremath{< 1} / $2043$ & \ensuremath{< 1} / $2043$ & MO / $5{\cdot} 10^{6}$ & \ensuremath{267} / $3{\cdot} 10^{6}$ & \ensuremath{279} / $3{\cdot} 10^{6}$ & 3 / $3{\cdot} 10^{5}$ & 3$^\dagger$ / $3{\cdot} 10^{5}$\\
\hline
maze2 & \multirow{2}{*}{Rmin} & \multirow{2}{*}{$15$} & \multirow{2}{*}{$8$} & \multirow{2}{*}{$54$} & \multirow{2}{*}{5.077} & $\le 5.692$ & $[5.692, 5.692]$ & $\ge 5.692$ & $\ge 5.692$ & $[5.692, 5.692]$ & $\ge 5.692$ & $\ge 5.692$ & $\ge 5.692$ & $\ge 5.692$\\
 &  &  &  &  &  & 2* / $26$ & \ensuremath{1.49} / $140$ & \ensuremath{< 1} / $27$ & \ensuremath{< 1} / $27$ & \ensuremath{3.02} / $6218$ & \ensuremath{< 1} / $23$ & \ensuremath{< 1} / $23$ & 8* / $23$ & 8* / $23$\\
\hline
maze2 & \multirow{2}{*}{Rmin} & \multirow{2}{*}{$16$} & \multirow{2}{*}{$8$} & \multirow{2}{*}{$58$} & \multirow{2}{*}{4.308} & $\le 5.624$ & $[5.247, 5.69]$ & $\ge 5.247$ & $\ge 5.247$ & $[5.624, 5.624]$ & $\ge 5.624$ & $\ge 5.624$ & $\ge 5.624$ & $\ge 5.624$\\
sl &  &  &  &  &  & 15 / $2{\cdot} 10^{6}$ & \ensuremath{1.48} / $150$ & \ensuremath{< 1} / $49$ & \ensuremath{< 1} / $49$ & \ensuremath{4.89} / $6296$ & \ensuremath{< 1} / $165$ & \ensuremath{< 1} / $165$ & 8* / $43$ & 8* / $43$\\
\hline
netw & \multirow{2}{*}{Rmin} & \multirow{2}{*}{$754$} & \multirow{2}{*}{$214$} & \multirow{2}{*}{$1218$} & \multirow{2}{*}{15.88} & $\le 19.32$ & $[18.76, 19.32]$ & $\ge 18.52$ & $\ge 18.52$ & $[19.24, 19.32]$ & $\ge 19.23$ & $\ge 19.23$ & $\ge 19.32$ & $\ge 19.32$\\
c2T2K20 &  &  &  &  &  & 9* / $4{\cdot} 10^{5}$ & \ensuremath{2.45} / $5831$ & \ensuremath{< 1} / $2720$ & \ensuremath{< 1} / $2720$ & \ensuremath{18} / $7{\cdot} 10^{4}$ & \ensuremath{< 1} / $9107$ & \ensuremath{< 1} / $9107$ & 10 / $2{\cdot} 10^{6}$ & 16* / $8{\cdot} 10^{6}$\\
\hline
netw & \multirow{2}{*}{Rmin} & \multirow{2}{*}{$677$} & \multirow{2}{*}{$214$} & \multirow{2}{*}{$833$} & \multirow{2}{*}{15.88} & $\le 19.32$ & $[18.76, 19.32]$ & $\ge 18.52$ & $\ge 18.52$ & $[19.24, 19.32]$ & $\ge 19.23$ & $\ge 19.23$ & $\ge 19.32$ & $\ge 19.32$\\
c2T2K20-ni &  &  &  &  &  & 6* / $3{\cdot} 10^{4}$ & \ensuremath{2.06} / $4311$ & \ensuremath{< 1} / $1834$ & \ensuremath{< 1} / $1834$ & \ensuremath{11.2} / $4{\cdot} 10^{4}$ & \ensuremath{< 1} / $5298$ & \ensuremath{< 1} / $5298$ & 16* / $5{\cdot} 10^{5}$ & 16* / $5{\cdot} 10^{5}$\\
\hline
netw & \multirow{2}{*}{Rmin} & \multirow{2}{*}{$2029$} & \multirow{2}{*}{$533$} & \multirow{2}{*}{$3133$} & \multirow{2}{*}{8.262} & $\le 10.29$ & $[9.851, 10.29]$ & $\ge 9.727$ & $\ge 9.727$ & $[10.2, 10.29]$ & $\ge 10.2$ & $\ge 10.2$ & $\ge 10.29$ & $\ge 10.29$\\
c2T4K20 &  &  &  &  &  & 10* / $2{\cdot} 10^{6}$ & \ensuremath{9.03} / $2{\cdot} 10^{4}$ & \ensuremath{< 1} / $7447$ & \ensuremath{< 1} / $7363$ & \ensuremath{112} / $2{\cdot} 10^{5}$ & \ensuremath{< 1} / $2{\cdot} 10^{4}$ & \ensuremath{< 1} / $2{\cdot} 10^{4}$ & 8 / $1{\cdot} 10^{6}$ & 12 / $1{\cdot} 10^{7}$\\
\hline
netw & \multirow{2}{*}{Rmin} & \multirow{2}{*}{$1832$} & \multirow{2}{*}{$533$} & \multirow{2}{*}{$2148$} & \multirow{2}{*}{8.262} & $\le 10.29$ & $[9.851, 10.29]$ & $\ge 9.727$ & $\ge 9.695$ & $[10.2, 10.29]$ & $\ge 10.2$ & $\ge 10.17$ & $\ge 10.29$ & $\ge 10.29$\\
c2T4K20-ni &  &  &  &  &  & 6* / $7{\cdot} 10^{4}$ & \ensuremath{6.71} / $1{\cdot} 10^{4}$ & \ensuremath{< 1} / $5092$ & \ensuremath{< 1} / $5076$ & \ensuremath{62.5} / $1{\cdot} 10^{5}$ & \ensuremath{< 1} / $1{\cdot} 10^{4}$ & \ensuremath{< 1} / $1{\cdot} 10^{4}$ & 11 / $7{\cdot} 10^{5}$ & 49 / $2{\cdot} 10^{6}$\\
\hline
netw & \multirow{2}{*}{Rmin} & \multirow{2}{*}{$4589$} & \multirow{2}{*}{$1173$} & \multirow{2}{*}{$6973$} & \multirow{2}{*}{2.557} & $\le 3.199$ & $[3.034, 3.199]$ & $\ge 2.965$ & $\ge 2.965$ & $[3.169, 3.199]$ & $\ge 3.171$ & $\ge 3.171$ & $\ge 3.199$ & $\ge 3.199$\\
c2T8K20 &  &  &  &  &  & 9 / $4{\cdot} 10^{6}$ & \ensuremath{37.1} / $4{\cdot} 10^{4}$ & \ensuremath{< 1} / $2{\cdot} 10^{4}$ & \ensuremath{< 1} / $2{\cdot} 10^{4}$ & \ensuremath{534} / $5{\cdot} 10^{5}$ & \ensuremath{< 1} / $5{\cdot} 10^{4}$ & \ensuremath{< 1} / $5{\cdot} 10^{4}$ & 8 / $2{\cdot} 10^{6}$ & 11 / $1{\cdot} 10^{7}$\\
\hline
netw & \multirow{2}{*}{Rmin} & \multirow{2}{*}{$4152$} & \multirow{2}{*}{$1173$} & \multirow{2}{*}{$4788$} & \multirow{2}{*}{2.557} & $\le 3.199$ & $[3.034, 3.199]$ & $\ge 2.965$ & $\ge 2.915$ & $[3.169, 3.199]$ & $\ge 3.171$ & $\ge 3.097$ & $\ge 3.199$ & $\ge 3.199$\\
c2T8K20-ni &  &  &  &  &  & 6* / $2{\cdot} 10^{5}$ & \ensuremath{27.9} / $3{\cdot} 10^{4}$ & \ensuremath{< 1} / $1{\cdot} 10^{4}$ & \ensuremath{< 1} / $1{\cdot} 10^{4}$ & \ensuremath{304} / $3{\cdot} 10^{5}$ & \ensuremath{< 1} / $3{\cdot} 10^{4}$ & \ensuremath{< 1} / $3{\cdot} 10^{4}$ & 10 / $1{\cdot} 10^{6}$ & 15 / $5{\cdot} 10^{6}$\\
\hline
netw & \multirow{2}{*}{Rmin} & \multirow{2}{*}{$1714$} & \multirow{2}{*}{$234$} & \multirow{2}{*}{$3154$} & \multirow{2}{*}{8.034} & $\le 13.74$ & $[10.68, 11.75]$ & $\ge 10.22$ & $\ge 10.22$ &  & $\ge 11.46$ & $\ge 11.46$ & $\ge 11.7$ & $\ge 11.73$\\
c3T3K8 &  &  &  &  &  & 8 / $2{\cdot} 10^{6}$ & \ensuremath{23.4} / $6{\cdot} 10^{4}$ & \ensuremath{< 1} / $1{\cdot} 10^{4}$ & \ensuremath{< 1} / $1{\cdot} 10^{4}$ & MO / $9{\cdot} 10^{6}$ & \ensuremath{1.55} / $8{\cdot} 10^{4}$ & \ensuremath{1.54} / $8{\cdot} 10^{4}$ & 5 / $8{\cdot} 10^{5}$ & 7$^\dagger$ / $7{\cdot} 10^{6}$\\
\hline
netw & \multirow{2}{*}{Rmin} & \multirow{2}{*}{$1625$} & \multirow{2}{*}{$234$} & \multirow{2}{*}{$2353$} & \multirow{2}{*}{8.034} & $\le 11.73$ & $[10.68, 11.75]$ & $\ge 10.22$ & $\ge 10.22$ & $[11.55, 11.74]$ & $\ge 11.46$ & $\ge 11.46$ & $\ge 11.72$ & $\ge 11.73$\\
c3T3K8-ni &  &  &  &  &  & 10* / $2{\cdot} 10^{6}$ & \ensuremath{18.1} / $5{\cdot} 10^{4}$ & \ensuremath{< 1} / $1{\cdot} 10^{4}$ & \ensuremath{< 1} / $1{\cdot} 10^{4}$ & \ensuremath{2527} / $6{\cdot} 10^{6}$ & \ensuremath{< 1} / $5{\cdot} 10^{4}$ & \ensuremath{< 1} / $5{\cdot} 10^{4}$ & 6 / $1{\cdot} 10^{6}$ & 9 / $1{\cdot} 10^{7}$\\
\hline
netw & \multirow{2}{*}{Rmin} & \multirow{2}{*}{$2729$} & \multirow{2}{*}{$361$} & \multirow{2}{*}{$4937$} & \multirow{2}{*}{5.73} & $\le 11.55$ & $[7.829, 8.88]$ & $\ge 7.427$ & $\ge 7.427$ &  & $\ge 8.592$ & $\ge 8.592$ & $\ge 8.826$ & $\ge 8.844$\\
c3T4K8 &  &  &  &  &  & 8 / $3{\cdot} 10^{6}$ & \ensuremath{52.5} / $1{\cdot} 10^{5}$ & \ensuremath{< 1} / $3{\cdot} 10^{4}$ & \ensuremath{< 1} / $2{\cdot} 10^{4}$ & MO / $2{\cdot} 10^{7}$ & \ensuremath{2.72} / $1{\cdot} 10^{5}$ & \ensuremath{2.72} / $1{\cdot} 10^{5}$ & 5 / $1{\cdot} 10^{6}$ & 7$^\dagger$ / $1{\cdot} 10^{7}$\\
\hline
netw & \multirow{2}{*}{Rmin} & \multirow{2}{*}{$2584$} & \multirow{2}{*}{$361$} & \multirow{2}{*}{$3632$} & \multirow{2}{*}{5.73} & $\le 9.091$ & $[7.829, 8.88]$ & $\ge 7.427$ & $\ge 7.427$ &  & $\ge 8.592$ & $\ge 8.592$ & $\ge 8.84$ & $\ge 8.844$\\
c3T4K8-ni &  &  &  &  &  & 8 / $3{\cdot} 10^{6}$ & \ensuremath{36.4} / $9{\cdot} 10^{4}$ & \ensuremath{< 1} / $2{\cdot} 10^{4}$ & \ensuremath{< 1} / $2{\cdot} 10^{4}$ & MO / $1{\cdot} 10^{7}$ & \ensuremath{1.32} / $8{\cdot} 10^{4}$ & \ensuremath{1.35} / $8{\cdot} 10^{4}$ & 6 / $2{\cdot} 10^{6}$ & 8$^\dagger$ / $1{\cdot} 10^{7}$\\
\hline
netw & \multirow{2}{*}{Rmin} & \multirow{2}{*}{$3753$} & \multirow{2}{*}{$489$} & \multirow{2}{*}{$6729$} & \multirow{2}{*}{4.162} & $\le 9.815$ & $[5.75, 6.714]$ & $\ge 5.42$ & $\ge 5.42$ &  & $\ge 6.429$ & $\ge 6.429$ & $\ge 6.615$ & $\ge 6.668$\\
c3T5K8 &  &  &  &  &  & 7 / $2{\cdot} 10^{6}$ & \ensuremath{89.9} / $1{\cdot} 10^{5}$ & \ensuremath{< 1} / $4{\cdot} 10^{4}$ & \ensuremath{< 1} / $4{\cdot} 10^{4}$ & MO / $2{\cdot} 10^{7}$ & \ensuremath{4.23} / $2{\cdot} 10^{5}$ & \ensuremath{4.2} / $2{\cdot} 10^{5}$ & 4 / $6{\cdot} 10^{5}$ & 7$^\dagger$ / $1{\cdot} 10^{7}$\\
\hline
netw & \multirow{2}{*}{Rmin} & \multirow{2}{*}{$3552$} & \multirow{2}{*}{$489$} & \multirow{2}{*}{$4920$} & \multirow{2}{*}{4.162} & $\le 7.005$ & $[5.75, 6.714]$ & $\ge 5.42$ & $\ge 5.418$ &  & $\ge 6.429$ & $\ge 6.419$ & $\ge 6.651$ & $\ge 6.669$\\
c3T5K8-ni &  &  &  &  &  & 8 / $4{\cdot} 10^{6}$ & \ensuremath{64.8} / $1{\cdot} 10^{5}$ & \ensuremath{< 1} / $3{\cdot} 10^{4}$ & \ensuremath{< 1} / $3{\cdot} 10^{4}$ & MO / $2{\cdot} 10^{7}$ & \ensuremath{1.92} / $1{\cdot} 10^{5}$ & \ensuremath{1.99} / $1{\cdot} 10^{5}$ & 5 / $9{\cdot} 10^{5}$ & 8$^\dagger$ / $1{\cdot} 10^{7}$\\
\hline
netw-prio & \multirow{2}{*}{Rmax} & \multirow{2}{*}{$1534$} & \multirow{2}{*}{$410$} & \multirow{2}{*}{$2782$} & \multirow{2}{*}{143} & $\ge 124.8$ & $[124.7, 127]$ & $\le 128.2$ & $\le 128.2$ & $[124.8, 125.1]$ & $\le 125.1$ & $\le 125.1$ & $\le 124.8$ & $\le 124.8$\\
c2T2K8 &  &  &  &  &  & 9* / $4{\cdot} 10^{5}$ & \ensuremath{6.17} / $1{\cdot} 10^{4}$ & \ensuremath{< 1} / $6116$ & \ensuremath{< 1} / $6114$ & \ensuremath{50} / $2{\cdot} 10^{5}$ & \ensuremath{< 1} / $2{\cdot} 10^{4}$ & \ensuremath{< 1} / $2{\cdot} 10^{4}$ & 8 / $1{\cdot} 10^{6}$ & 11 / $7{\cdot} 10^{6}$\\
\hline
netw-prio & \multirow{2}{*}{Rmax} & \multirow{2}{*}{$1959$} & \multirow{2}{*}{$702$} & \multirow{2}{*}{$2667$} & \multirow{2}{*}{143} & $\ge 124.6$ & $[124.5, 127.7]$ & $\le 127.6$ & $\le 127.6$ & $[124.6, 125]$ & $\le 125$ & $\le 125$ & $\le 124.6$ & $\le 124.6$\\
c2T2K8-ni &  &  &  &  &  & 4* / $3{\cdot} 10^{4}$ & \ensuremath{6.49} / $1{\cdot} 10^{4}$ & \ensuremath{< 1} / $4151$ & \ensuremath{< 1} / $4151$ & \ensuremath{49.1} / $1{\cdot} 10^{5}$ & \ensuremath{< 1} / $1{\cdot} 10^{4}$ & \ensuremath{< 1} / $1{\cdot} 10^{4}$ & 13 / $4{\cdot} 10^{5}$ & 20 / $6{\cdot} 10^{5}$\\
\hline
netw-prio & \multirow{2}{*}{Rmax} & \multirow{2}{*}{$3577$} & \multirow{2}{*}{$921$} & \multirow{2}{*}{$6361$} & \multirow{2}{*}{191.3} & $\ge 179.9$ & $[179.8, 182.1]$ & $\le 183.1$ & $\le 183.1$ & $[179.9, 180.3]$ & $\le 180.3$ & $\le 180.3$ & $\le 179.9$ & $\le 179.9$\\
c2T4K8 &  &  &  &  &  & 10* / $2{\cdot} 10^{6}$ & \ensuremath{22.9} / $3{\cdot} 10^{4}$ & \ensuremath{< 1} / $1{\cdot} 10^{4}$ & \ensuremath{< 1} / $1{\cdot} 10^{4}$ & \ensuremath{198} / $4{\cdot} 10^{5}$ & \ensuremath{< 1} / $5{\cdot} 10^{4}$ & \ensuremath{< 1} / $5{\cdot} 10^{4}$ & 7 / $1{\cdot} 10^{6}$ & 10 / $1{\cdot} 10^{7}$\\
\hline
netw-prio & \multirow{2}{*}{Rmax} & \multirow{2}{*}{$5498$} & \multirow{2}{*}{$1721$} & \multirow{2}{*}{$7226$} & \multirow{2}{*}{191.3} & $\ge 171$ & $[170.7, 174.7]$ & $\le 174.5$ & $\le 174.5$ & $[170.9, 171.8]$ & $\le 171.5$ & $\le 171.5$ & $\le 171$ & $\le 171$\\
c2T4K8-ni &  &  &  &  &  & 5* / $9{\cdot} 10^{4}$ & \ensuremath{34.9} / $4{\cdot} 10^{4}$ & \ensuremath{< 1} / $1{\cdot} 10^{4}$ & \ensuremath{< 1} / $1{\cdot} 10^{4}$ & \ensuremath{271} / $5{\cdot} 10^{5}$ & \ensuremath{< 1} / $3{\cdot} 10^{4}$ & \ensuremath{< 1} / $3{\cdot} 10^{4}$ & 11 / $1{\cdot} 10^{6}$ & 15 / $3{\cdot} 10^{6}$\\
\hline
netw-prio & \multirow{2}{*}{Rmax} & \multirow{2}{*}{$7673$} & \multirow{2}{*}{$1945$} & \multirow{2}{*}{$1{\cdot} 10^{4}$} & \multirow{2}{*}{225.9} & $\ge 213$ & $[222.2, 223.1]$ & $\le 223.5$ & $\le 223.5$ & $[222.2, 222.4]$ & $\le 222.4$ & $\le 222.4$ & $\le 222.3$ & $\le 222.3$\\
c2T8K8 &  &  &  &  &  & 8 / $4{\cdot} 10^{6}$ & \ensuremath{75.9} / $7{\cdot} 10^{4}$ & \ensuremath{< 1} / $3{\cdot} 10^{4}$ & \ensuremath{< 1} / $3{\cdot} 10^{4}$ & \ensuremath{799} / $9{\cdot} 10^{5}$ & \ensuremath{1.45} / $9{\cdot} 10^{4}$ & \ensuremath{1.52} / $9{\cdot} 10^{4}$ & 6 / $1{\cdot} 10^{6}$ & 10 / $2{\cdot} 10^{7}$\\
\hline
netw-prio & \multirow{2}{*}{Rmax} & \multirow{2}{*}{$1{\cdot} 10^{4}$} & \multirow{2}{*}{$3769$} & \multirow{2}{*}{$2{\cdot} 10^{4}$} & \multirow{2}{*}{225.9} & $\ge 196.6$ & $[196.2, 199.6]$ & $\le 199.5$ & $\le 199.5$ & $[196.5, 197.7]$ & $\le 197.4$ & $\le 197.4$ & $\le 196.6$ & $\le 196.6$\\
c2T8K8-ni &  &  &  &  &  & 5* / $4{\cdot} 10^{5}$ & \ensuremath{157} / $9{\cdot} 10^{4}$ & \ensuremath{< 1} / $3{\cdot} 10^{4}$ & \ensuremath{< 1} / $3{\cdot} 10^{4}$ & \ensuremath{1253} / $1{\cdot} 10^{6}$ & \ensuremath{1.61} / $7{\cdot} 10^{4}$ & \ensuremath{1.57} / $7{\cdot} 10^{4}$ & 9 / $1{\cdot} 10^{6}$ & 14 / $6{\cdot} 10^{6}$\\
\hline
netw-prio & \multirow{2}{*}{Rmax} & \multirow{2}{*}{$3932$} & \multirow{2}{*}{$524$} & \multirow{2}{*}{$8540$} & \multirow{2}{*}{56.84} & $\ge 44.18$ & $[44.11, 47.17]$ & $\le 49.36$ & $\le 49.36$ &  & $\le 44.75$ & $\le 44.75$ & $\le 44.44$ & $\le 44.18$\\
c3T3K2 &  &  &  &  &  & 5* / $2{\cdot} 10^{5}$ & \ensuremath{94.5} / $1{\cdot} 10^{5}$ & \ensuremath{1.55} / $2{\cdot} 10^{4}$ & \ensuremath{1.47} / $2{\cdot} 10^{4}$ & MO / $2{\cdot} 10^{7}$ & \ensuremath{4.61} / $1{\cdot} 10^{5}$ & \ensuremath{5.02} / $1{\cdot} 10^{5}$ & 4 / $4{\cdot} 10^{5}$ & 24* / $7{\cdot} 10^{6}$\\
\hline
netw-prio & \multirow{2}{*}{Rmax} & \multirow{2}{*}{$3707$} & \multirow{2}{*}{$524$} & \multirow{2}{*}{$6515$} & \multirow{2}{*}{56.84} & $\ge 44.18$ & $[44.11, 47.17]$ & $\le 49.36$ & $\le 49.36$ &  & $\le 44.75$ & $\le 44.75$ & $\le 44.3$ & $\le 44.18$\\
c3T3K2-ni &  &  &  &  &  & 4* / $7{\cdot} 10^{4}$ & \ensuremath{66.5} / $1{\cdot} 10^{5}$ & \ensuremath{< 1} / $2{\cdot} 10^{4}$ & \ensuremath{< 1} / $2{\cdot} 10^{4}$ & MO / $1{\cdot} 10^{7}$ & \ensuremath{2.78} / $7{\cdot} 10^{4}$ & \ensuremath{2.62} / $7{\cdot} 10^{4}$ & 5 / $7{\cdot} 10^{5}$ & 24 / $3{\cdot} 10^{6}$\\
\hline
netw-prio & \multirow{2}{*}{Rmax} & \multirow{2}{*}{$5971$} & \multirow{2}{*}{$779$} & \multirow{2}{*}{$1{\cdot} 10^{4}$} & \multirow{2}{*}{67.02} & $\ge 55.64$ & $[55.47, 58.92]$ & $\le 60.91$ & $\le 60.91$ &  & $\le 56.26$ & $\le 56.26$ & $\le 55.95$ & $\le 55.64$\\
c3T4K2 &  &  &  &  &  & 7* / $1{\cdot} 10^{6}$ & \ensuremath{193} / $2{\cdot} 10^{5}$ & \ensuremath{2.51} / $4{\cdot} 10^{4}$ & \ensuremath{2.5} / $4{\cdot} 10^{4}$ & MO / $3{\cdot} 10^{7}$ & \ensuremath{12.5} / $2{\cdot} 10^{5}$ & \ensuremath{13} / $2{\cdot} 10^{5}$ & 4 / $8{\cdot} 10^{5}$ & 7$^\dagger$ / $2{\cdot} 10^{7}$\\
\hline
netw-prio & \multirow{2}{*}{Rmax} & \multirow{2}{*}{$5620$} & \multirow{2}{*}{$779$} & \multirow{2}{*}{$9724$} & \multirow{2}{*}{67.02} & $\ge 55.63$ & $[55.46, 58.91]$ & $\le 60.91$ & $\le 60.91$ &  & $\le 56.26$ & $\le 56.26$ & $\le 55.94$ & $\le 55.63$\\
c3T4K2-ni &  &  &  &  &  & 6* / $4{\cdot} 10^{5}$ & \ensuremath{128} / $2{\cdot} 10^{5}$ & \ensuremath{1.43} / $3{\cdot} 10^{4}$ & \ensuremath{1.4} / $3{\cdot} 10^{4}$ & MO / $2{\cdot} 10^{7}$ & \ensuremath{5.62} / $1{\cdot} 10^{5}$ & \ensuremath{5.91} / $1{\cdot} 10^{5}$ & 4 / $5{\cdot} 10^{5}$ & 9$^\dagger$ / $2{\cdot} 10^{7}$\\
\hline
netw-prio & \multirow{2}{*}{Rmax} & \multirow{2}{*}{$8019$} & \multirow{2}{*}{$1035$} & \multirow{2}{*}{$2{\cdot} 10^{4}$} & \multirow{2}{*}{73.57} & $\ge 60.72$ & $[64.09, 67.4]$ & $\le 69.04$ & $\le 69.04$ &  & $\le 64.97$ & $\le 64.97$ & $\le 65.2$ & $\le 64.31$\\
c3T5K2 &  &  &  &  &  & 5 / $1{\cdot} 10^{6}$ & \ensuremath{305} / $3{\cdot} 10^{5}$ & \ensuremath{3.08} / $7{\cdot} 10^{4}$ & \ensuremath{3.06} / $7{\cdot} 10^{4}$ & MO / $5{\cdot} 10^{7}$ & \ensuremath{20.8} / $4{\cdot} 10^{5}$ & \ensuremath{20.8} / $4{\cdot} 10^{5}$ & 3 / $4{\cdot} 10^{5}$ & 6$^\dagger$ / $1{\cdot} 10^{7}$\\
\hline
netw-prio & \multirow{2}{*}{Rmax} & \multirow{2}{*}{$7542$} & \multirow{2}{*}{$1035$} & \multirow{2}{*}{$1{\cdot} 10^{4}$} & \multirow{2}{*}{73.57} & $\ge 64.29$ & $[64.09, 67.4]$ & $\le 69.03$ & $\le 69.03$ &  & $\le 64.96$ & $\le 64.96$ & $\le 64.48$ & $\le 64.29$\\
c3T5K2-ni &  &  &  &  &  & 7* / $1{\cdot} 10^{6}$ & \ensuremath{216} / $3{\cdot} 10^{5}$ & \ensuremath{1.7} / $5{\cdot} 10^{4}$ & \ensuremath{1.71} / $5{\cdot} 10^{4}$ & MO / $3{\cdot} 10^{7}$ & \ensuremath{8.59} / $2{\cdot} 10^{5}$ & \ensuremath{8.29} / $2{\cdot} 10^{5}$ & 4 / $7{\cdot} 10^{5}$ & 7$^\dagger$ / $1{\cdot} 10^{7}$\\
\hline
ngrid & \multirow{2}{*}{Pmax} & \multirow{2}{*}{$19$} & \multirow{2}{*}{$4$} & \multirow{2}{*}{$67$} & \multirow{2}{*}{1} & $\ge 1$ & $[0, 1]$ & $\le 1$ & $\le 1$ &  & $\le 1$ & $\le 1$ & $\le 1$ & $\le 1$\\
N3 &  &  &  &  &  & 1* / $114$ & \ensuremath{1.86} / $3878$ & \ensuremath{< 1} / $114$ & \ensuremath{< 1} / $89$ & MO / $2{\cdot} 10^{7}$ & \ensuremath{< 1} / $114$ & \ensuremath{< 1} / $89$ & 4* / $114$ & 4* / $114$\\
\hline
ngrid & \multirow{2}{*}{Pmax} & \multirow{2}{*}{$28$} & \multirow{2}{*}{$4$} & \multirow{2}{*}{$103$} & \multirow{2}{*}{1} & $\ge 1$ & $[0, 1]$ & $\le 1$ & $\le 1$ &  & $\le 1$ & $\le 1$ & $\le 1$ & $\le 1$\\
N4 &  &  &  &  &  & 1* / $231$ & \ensuremath{12.5} / $2{\cdot} 10^{4}$ & \ensuremath{< 1} / $231$ & \ensuremath{< 1} / $137$ & MO / N/A & \ensuremath{< 1} / $231$ & \ensuremath{< 1} / $137$ & 4* / $231$ & 4* / $231$\\
\hline
ngrid & \multirow{2}{*}{Pmax} & \multirow{2}{*}{$39$} & \multirow{2}{*}{$4$} & \multirow{2}{*}{$147$} & \multirow{2}{*}{1} & $\ge 1$ & $[0, 1]$ & $\le 1$ & $\le 1$ &  & $\le 1$ & $\le 1$ & $\le 1$ & $\le 1$\\
N5 &  &  &  &  &  & 1* / $379$ & \ensuremath{91.3} / $8{\cdot} 10^{4}$ & \ensuremath{< 1} / $379$ & \ensuremath{< 1} / $269$ & MO / N/A & \ensuremath{< 1} / $379$ & \ensuremath{< 1} / $269$ & 4* / $379$ & 4* / $379$\\
\hline
ngrid & \multirow{2}{*}{Pmax} & \multirow{2}{*}{$52$} & \multirow{2}{*}{$4$} & \multirow{2}{*}{$199$} & \multirow{2}{*}{1} & $\ge 1$ & $[0, 1]$ & $\le 1$ & $\le 1$ &  & $\le 1$ & $\le 1$ & $\le 1$ & $\le 1$\\
N6 &  &  &  &  &  & 1* / $586$ & \ensuremath{554} / $3{\cdot} 10^{5}$ & \ensuremath{< 1} / $586$ & \ensuremath{< 1} / $495$ & MO / N/A & \ensuremath{< 1} / $586$ & \ensuremath{< 1} / $495$ & 3* / $586$ & 3* / $586$\\
\hline
refuel & \multirow{2}{*}{Pmax} & \multirow{2}{*}{$126$} & \multirow{2}{*}{$39$} & \multirow{2}{*}{$319$} & \multirow{2}{*}{0.904} & $\ge 0.487$ &  & $\le 0.592$ & $\le 0.592$ &  & $\le 0.498$ & $\le 0.498$ & $\le 0.487$ & $\le 0.487$\\
N05 &  &  &  &  &  & 12 / $3{\cdot} 10^{6}$ & NS / N/A & \ensuremath{< 1} / $883$ & \ensuremath{< 1} / $863$ & NS / N/A & \ensuremath{< 1} / $5351$ & \ensuremath{< 1} / $5184$ & 12* / $5{\cdot} 10^{5}$ & 12* / $5{\cdot} 10^{5}$\\
\hline
refuel & \multirow{2}{*}{Pmax} & \multirow{2}{*}{$208$} & \multirow{2}{*}{$50$} & \multirow{2}{*}{$565$} & \multirow{2}{*}{0.981} & $\ge 0.672$ &  & $\le 0.713$ & $\le 0.713$ &  & $\le 0.677$ & $\le 0.677$ & $\le 0.672$ & $\le 0.672$\\
N06 &  &  &  &  &  & 10 / $2{\cdot} 10^{6}$ & NS / N/A & \ensuremath{< 1} / $5866$ & \ensuremath{< 1} / $5614$ & NS / N/A & \ensuremath{2.63} / $2{\cdot} 10^{5}$ & \ensuremath{2.5} / $2{\cdot} 10^{5}$ & 11* / $1{\cdot} 10^{4}$ & 11* / $1{\cdot} 10^{4}$\\
\hline
refuel & \multirow{2}{*}{Pmax} & \multirow{2}{*}{$322$} & \multirow{2}{*}{$55$} & \multirow{2}{*}{$941$} & \multirow{2}{*}{0.961} & $\ge 0.506$ &  & $\le 0.682$ & $\le 0.682$ &  & $\le 0.562$ & $\le 0.562$ & $\le 0.586$ & $\le 0.586$\\
N07 &  &  &  &  &  & 8 / $1{\cdot} 10^{6}$ & NS / N/A & \ensuremath{< 1} / $2{\cdot} 10^{4}$ & \ensuremath{< 1} / $2{\cdot} 10^{4}$ & NS / N/A & \ensuremath{94.5} / $4{\cdot} 10^{6}$ & \ensuremath{98.6} / $3{\cdot} 10^{6}$ & 3 / $2{\cdot} 10^{6}$ & 3$^\dagger$ / $2{\cdot} 10^{6}$\\
\hline
refuel & \multirow{2}{*}{Pmax} & \multirow{2}{*}{$470$} & \multirow{2}{*}{$66$} & \multirow{2}{*}{$1431$} & \multirow{2}{*}{0.989} & $\ge 0.446$ &  & $\le 0.759$ & $\le 0.759$ &  &  &  & $\le 0.749$ & $\le 0.483$\\
N08 &  &  &  &  &  & 7 / $1{\cdot} 10^{6}$ & NS / N/A & \ensuremath{7.28} / $1{\cdot} 10^{5}$ & \ensuremath{7.28} / $1{\cdot} 10^{5}$ & NS / N/A & MO / N/A & MO / N/A & 2 / $1{\cdot} 10^{5}$ & 3$^\dagger$ / $1{\cdot} 10^{6}$\\
\hline
refuel & \multirow{2}{*}{Pmax} & \multirow{2}{*}{$672$} & \multirow{2}{*}{$75$} & \multirow{2}{*}{$2121$} & \multirow{2}{*}{0.989} & $\ge 0.434$ &  & $\le 0.737$ & $\le 0.737$ &  &  &  & $\le 0.769$ & $\le 0.769$\\
N09 &  &  &  &  &  & 7 / $3{\cdot} 10^{6}$ & NS / N/A & \ensuremath{13.8} / $4{\cdot} 10^{5}$ & \ensuremath{13.6} / $4{\cdot} 10^{5}$ & NS / N/A & MO / N/A & MO / N/A & 2 / $4{\cdot} 10^{5}$ & 3$^\dagger$ / $5{\cdot} 10^{6}$\\
\hline
refuel & \multirow{2}{*}{Pmax} & \multirow{2}{*}{$892$} & \multirow{2}{*}{$84$} & \multirow{2}{*}{$2879$} & \multirow{2}{*}{0.998} & $\ge 0.425$ &  & $\le 0.838$ & $\le 0.838$ &  &  &  & $\le 0.868$ & $\le 0.868$\\
N10 &  &  &  &  &  & 5 / $1{\cdot} 10^{6}$ & NS / N/A & \ensuremath{46.7} / $1{\cdot} 10^{6}$ & \ensuremath{46.8} / $9{\cdot} 10^{5}$ & NS / N/A & MO / N/A & MO / N/A & 1 / $1{\cdot} 10^{5}$ & 2$^\dagger$ / $1{\cdot} 10^{6}$\\
\hline
repud & \multirow{2}{*}{Pmax} & \multirow{2}{*}{$39$} & \multirow{2}{*}{$21$} & \multirow{2}{*}{$49$} & \multirow{2}{*}{1} & $\ge 0.25$ & $[0.25, 0.375]$ & $\le 0.25$ & $\le 0.25$ & $[0.25, 0.25]$ & $\le 0.25$ & $\le 0.25$ & $\le 0.25$ & $\le 0.25$\\
K4 &  &  &  &  &  & 2* / $26$ & \ensuremath{1.48} / $173$ & \ensuremath{< 1} / $16$ & \ensuremath{< 1} / $16$ & \ensuremath{1.49} / $1685$ & \ensuremath{< 1} / $16$ & \ensuremath{< 1} / $16$ & 3* / $19$ & 3* / $19$\\
\hline
repud & \multirow{2}{*}{Pmax} & \multirow{2}{*}{$125$} & \multirow{2}{*}{$41$} & \multirow{2}{*}{$161$} & \multirow{2}{*}{1} & $\ge 0.125$ & $[0.125, 0.375]$ & $\le 0.25$ & $\le 0.25$ & $[0.125, 0.221]$ & $\le 0.125$ & $\le 0.125$ & $\le 0.125$ & $\le 0.125$\\
K8 &  &  &  &  &  & 2* / $52$ & \ensuremath{1.53} / $2385$ & \ensuremath{< 1} / $53$ & \ensuremath{< 1} / $53$ & \ensuremath{22.6} / $2{\cdot} 10^{5}$ & \ensuremath{< 1} / $32$ & \ensuremath{< 1} / $32$ & 6* / $45$ & 6* / $45$\\
\hline
samplerocks & \multirow{2}{*}{Rmin} & \multirow{2}{*}{$1081$} & \multirow{2}{*}{$277$} & \multirow{2}{*}{$4465$} & \multirow{2}{*}{5.5} & $\le 8.492$ &  & $\ge 8$ & $\ge 8$ &  & $\ge 8$ & $\ge 8$ & $\ge 8$ & $\ge 8$\\
N04 &  &  &  &  &  & 8 / $6{\cdot} 10^{5}$ & NS / N/A & \ensuremath{< 1} / $1{\cdot} 10^{4}$ & \ensuremath{< 1} / $1{\cdot} 10^{4}$ & NS / N/A & \ensuremath{8.35} / $3{\cdot} 10^{5}$ & \ensuremath{8.34} / $3{\cdot} 10^{5}$ & 8* / $6199$ & 8* / $6199$\\
\hline
samplerocks & \multirow{2}{*}{Rmin} & \multirow{2}{*}{$3241$} & \multirow{2}{*}{$817$} & \multirow{2}{*}{$1{\cdot} 10^{4}$} & \multirow{2}{*}{11} & $\le 38$ &  & $\ge 14$ & $\ge 14$ &  & $\ge 14$ & $\ge 14$ & $\ge 14$ & $\ge 14$\\
N08 &  &  &  &  &  & 7 / $8{\cdot} 10^{5}$ & NS / N/A & \ensuremath{< 1} / $3{\cdot} 10^{4}$ & \ensuremath{< 1} / $3{\cdot} 10^{4}$ & NS / N/A & \ensuremath{36.1} / $9{\cdot} 10^{5}$ & \ensuremath{35.9} / $9{\cdot} 10^{5}$ & 8* / $2{\cdot} 10^{4}$ & 8* / $2{\cdot} 10^{4}$\\
\hline
samplerocks & \multirow{2}{*}{Rmin} & \multirow{2}{*}{$6553$} & \multirow{2}{*}{$1645$} & \multirow{2}{*}{$3{\cdot} 10^{4}$} & \multirow{2}{*}{16.5} & $\le 208.5$ &  & $\ge 19.9$ & $\ge 19.9$ &  & $\ge 20$ & $\ge 20$ & $\ge 20$ & $\ge 20$\\
N12 &  &  &  &  &  & 6 / $8{\cdot} 10^{5}$ & NS / N/A & \ensuremath{1.76} / $7{\cdot} 10^{4}$ & \ensuremath{1.76} / $7{\cdot} 10^{4}$ & NS / N/A & \ensuremath{86.7} / $2{\cdot} 10^{6}$ & \ensuremath{88.1} / $2{\cdot} 10^{6}$ & 10* / $1{\cdot} 10^{5}$ & 10* / $1{\cdot} 10^{5}$\\
\hline
samplerocks & \multirow{2}{*}{Rmin} & \multirow{2}{*}{$1{\cdot} 10^{4}$} & \multirow{2}{*}{$2761$} & \multirow{2}{*}{$5{\cdot} 10^{4}$} & \multirow{2}{*}{22} & $\le 370.9$ &  & $\ge 25.6$ & $\ge 25.6$ &  & $\ge 26$ & $\ge 26$ & $\ge 25.74$ & $\ge 25.86$\\
N16 &  &  &  &  &  & 5 / $7{\cdot} 10^{5}$ & NS / N/A & \ensuremath{3.77} / $1{\cdot} 10^{5}$ & \ensuremath{3.83} / $1{\cdot} 10^{5}$ & NS / N/A & \ensuremath{166} / $3{\cdot} 10^{6}$ & \ensuremath{164} / $3{\cdot} 10^{6}$ & 7 / $4{\cdot} 10^{5}$ & 10$^\dagger$ / $3{\cdot} 10^{6}$\\
\hline
samplerocks & \multirow{2}{*}{Rmin} & \multirow{2}{*}{$4{\cdot} 10^{4}$} & \multirow{2}{*}{$1{\cdot} 10^{4}$} & \multirow{2}{*}{$2{\cdot} 10^{5}$} & \multirow{2}{*}{44} & $\le 1750$ &  & $\ge 47.67$ & $\ge 47.67$ &  & $\ge 49.85$ & $\ge 49.85$ & $\ge 47.57$ & $\ge 48.11$\\
N32 &  &  &  &  &  & 3 / $6{\cdot} 10^{5}$ & NS / N/A & \ensuremath{38} / $4{\cdot} 10^{5}$ & \ensuremath{34.1} / $4{\cdot} 10^{5}$ & NS / N/A & \ensuremath{1391} / $1{\cdot} 10^{7}$ & \ensuremath{1436} / $1{\cdot} 10^{7}$ & 6 / $2{\cdot} 10^{5}$ & 10$^\dagger$ / $2{\cdot} 10^{6}$\\
\hline
\end{tabular}


==> preliminaries.tex <==
%!TEX root = main.tex
% !TeX spellcheck = en_GB



%\subsection*{Further notation}
\sj{In the latex source there are additional definitions}

%
%\paragraph{Geometry}
%We write $\rrnn = \set{|x| \mid x \in \rr}$ and $\rrinf = \rr \cup \set{\infty}$ for the non-negative and extended real numbers, respectively.
%%Let $\tupleaccess{\vertex}{i}$ denote the $i^\mathrm{th}$ entry of $\vertex \in \rr^\numstates$.
%
%An $\numstates$-dimensional halfspace with normal vector $\vect \in \rr^\numstates$ and offset $b \in \rr$ is a set $\halfspace = \set{ \vec{x} \in \rr^\numstates \mid \vect \cdot \vec{x} \triangleleft b}$, where ${\triangleleft} \in \set{{<}, {\le}}$.
%A polytope $\polytope$ is an intersection of finitely many (closed or open) halfspaces.
%A halfspace $\halfspace$ is called closed if $\triangleleft = \le$ and open otherwise.
%A Similarly, a polytope is closed if it is the intersection of closed halfspaces.
%The closure $\clof{\polytope}$ of a polytope $\polytope$ is obtained by replacing open halfspaces in the intersection with closed ones.
%A polytope $\polytope$ is bounded if $\ex{y \in \rr^\numstates} \fa{\tuple{x_1, \dots, x_\numstates} \in \polytope} \fa{i} |x_i| \le y$.
%
%The convex closure of a set $\points \subseteq \rr^\numstates$ is given by
%$\conv{\points} = \{\beliefstate \in \rr^\numstates \mid  \ex{\vertex_1,\dots,\vertex_\numstates \in \rr^\numstates, \dist \in \dists{\set{\vertex_1, \dots, \vertex_\numstates}}}   \sum_i \dist(\vertex_i) \cdot \vertex_i = \beliefstate \}$.
%We say that $\points$ is \emph{convex} if $\points = \conv{\points}$.
%Polytopes are always convex.
%For a bounded polytope $\polytope$ there is a finite set of points $\points \subseteq \rr^\numstates$ whose convex closure coincides with the closure of $\polytope$. 
%We call the smallest such set the \emph{vertices} of $\polytope$, denoted by $\vertices{\polytope}$.


